Accurate and Fast Approximate Graph Pattern Mining at Scale

Approximate graph pattern mining (A-GPM) is an important data analysis tool for many graph-based applications. There exist sampling-based A-GPM systems to provide automation and generalization over a wide variety of use cases. However, there are two major obstacles that prevent existing A-GPM systems being adopted in practice. First, the termination mechanism that decides when to end sampling lacks theoretical backup on confidence, and is unstable and slow in practice. Second, they suffer poor performance when dealing with the "needle-in-the-hay" cases, because a huge number of samples are required to converge, given the extremely low hit rate of their fixed sampling schemes. We build ScaleGPM, an accurate and fast A-GPM system that removes the two obstacles. First, we propose a novel on-the-fly convergence detection mechanism to achieve stable termination and provide theoretical guarantee on the confidence, with negligible overhead. Second, we propose two techniques to deal with the "needle-in-the-hay" problem, eager-verify and hybrid sampling. Our eager-verify method improves sampling hit rate by pruning unpromising candidates as early as possible. Hybrid sampling improves performance by automatically choosing the better scheme between fine-grained and coarse-grained sampling schemes. Experiments show that our online convergence detection mechanism can detect convergence and results in stable and rapid termination with theoretically guaranteed confidence. We show the effectiveness of eager-verify in improving the hit rate, and the scheme-selection mechanism in correctly choosing the better scheme for various cases. Overall, ScaleGPM achieves a geomean average of 565x (up to 610169x) speedup over the state-of-the-art A-GPM system, Arya. In particular, ScaleGPM handles billion-scale graphs in seconds, where existing systems either run out of memory or fail to complete in hours.

==> algo-ELP.tex <==
%ELP Algorithm%
\iffalse
\begin{algorithm}[tb]
\footnotesize
\caption{Error Latency Profile for Sparsification}
\label{alg1:spar}
\begin{algorithmic}[1]

% \Input
% \State \makebox[4em][l]{$G(V,E)$} data graph
% \State \makebox[4em][l]{$P$} pattern graph
% \State \makebox[4em][l]{$\epsilon$} error bound
% \State \makebox[4em][l]{$p$} sample fraction
% \State \makebox[4em][l]{$\delta$} maximum number of colors to support
% \EndInput

% \Output
% \State \makebox[4em][l] {$C$} a $c$, for the number of colors to use in the graph.
% \EndOutput

\State {$G' \leftarrow \Call{EdgeSparsify}{\mathcal{G},p}$}
\State {$G_c \leftarrow \Call{Color}{\mathcal{G},\delta,3}$}

\While {$\texttt{true}$}
    \State {Run Sansa 3 times with the three unique coloring in $G_c$ for $N_c$}
    \State {$avg_{cur} \leftarrow$ \text{the average count of the 3 trials}}
    \State{$range_{cur} \leftarrow \text{the range (max-min) of the 3 trials.}$}
    \State{$\epsilon' \leftarrow \vert avg_{last} - avg_{cur}\vert / avg_cur$}

    \If {$\frac{range_{last}}{avg_{last}} \le 10\% \text{and} \epsilon' < \epsilon \text{and} \frac{range_{cur}}{avg_{cur}} < 10\%$}
        \State {$C \leftarrow N_c$}
        \State {$h \leftarrow avg_{cur}$}
        \State {$\texttt{Break}$}
    \EndIf

   \State{$ N_c \leftarrow N_c / 2, avg_{cur} \leftarrow avg_{cur}, range_{last} \leftarrow range_{cur}$} 
\EndWhile
\end{algorithmic}
\end{algorithm}
\fi

%ELP Algorithm%
\newcommand{\algorithmicbreak}{\textbf{break}}
\newcommand{\Break}{\State \algorithmicbreak}
\newcommand{\algorithmicand}{\textbf{and}}
\newcommand{\AND}{\algorithmicand}

\begin{algorithm}[tb]
\footnotesize
\caption{Fast Profiling}
\label{algo:elp}
\begin{algorithmic}[1]
%\Input
%\State \makebox[4em][l]{$G(V,E)$} data graph
%\State \makebox[4em][l]{$P$} pattern graph
%\State \makebox[4em][l]{$\epsilon$} error bound
%\State \makebox[4em][l]{$p$} sample fraction
%\State \makebox[4em][l]{$\delta$} maximum number of colors to support
%\EndInput

%\Output
%\State \makebox[4em][l] {$C$} a $c$, for the number of colors to use in the graph.
%\EndOutput

\Procedure{Profiling}{\dg, \pg, $\epsilon, \delta, R_0$}
%\State $ N_0 \gets R_0.N_s, W_0 \gets R_0.W$

\State $es \gets$\Call{SampleEdges}{\dg, $p$}
\State $G' \gets$ \Call{GenSubgraph}{\dg, $es$}, 
 $C \gets 0, r \gets 0$, $\tilde{\epsilon} \gets 0$ %\Comment{ELP aims to roughly estimate the exact count $C$}
\While {$\texttt{true}$}
    \For{$i : [1,N]$} %\Comment{$N = 3$}
    \State $H_i \gets$ \Call{\hlg{Sample}}{$G'$, \pg, $R_0$}  \Comment{UDF}
    %\State $H_i \gets$ \Call{\hlg{NS-Engine}}{$G'$, \pg, $R_0$}  \Comment{UDF}
    \State $C_i \gets$ \Call{\hlg{Count}}{$H_i$, \pg}  \Comment{UDF}
    \EndFor
    \State $C' \gets \sum C_i / N$, $r' \gets$ \Call{Max}{$C_i$} $-$ \Call{Min}{$C_i$}, 
    $\tilde{\epsilon} \gets \frac{|C - C'|}{C'}$ 
    \If {
         $\tilde{\epsilon} < \epsilon$ \AND \ 
         $\frac{r'}{C'} < \eta$ \AND \ 
         $\frac{r}{C} < \eta$} \Comment{$\eta = 0.1$
        }
        %\State {$C \gets N_c$}
        %\State {$h \gets C'$}
        \Break
    \EndIf
    \State $R_0 \gets$ \Call{\hlg{AdjustSamplingRule}}{$R_0$} \Comment{UDF}
    \State $C \gets C', r \gets r'$ 
\EndWhile
\State \Return \Call{\hlg{GenSamplingRule}}{\dg, \pg, $\epsilon$, $\delta$, $R_0$, $\dots$}  \Comment{UDF}
\EndProcedure
\end{algorithmic}
\end{algorithm}

% \begin{algorithm}[tb]
% \footnotesize
% \caption{Generate Scaling Factor}
% \label{algo:scale}
% \begin{algorithmic}[1]
% \Procedure{GenScaleFactor}{$\mathcal{G}, P$}
% \State 
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

==> algo-color.tex <==
\begin{algorithm}[tb]
\footnotesize
\caption{Color sparsification}
\label{alg1:main}
\begin{algorithmic}[1]

%Color Sparsification Algorithm%

\Input
\State \makebox[4em][l]{$G(V,E)$} data graph
\State \makebox[4em][l]{$\delta$} max number of colors
\State \makebox[4em][l]{$\k$} number of colors to pre-generate / store at a time
\EndInput

\Output
\State \makebox[4em][l] {$G_c$} color sparsified graph of g
\EndOutput



%\tikzmk{A}
\For{{\bf each} $ v \in$ $V$ \textbf{}}
\State $colors[v][i] = rand(0,delta) \vert$ for $i$ in [0,$k$]  
\EndFor
%\tikzmk{B} \boxit{blue}

%\tikzmk{A}
%\For{{\bf each} color $ i \in$ $[0,k)$ \textbf{}}
\State count += \Call{ExactCounting}{$\mathcal{G}_i$, $P$} \Comment{\hl{Exact counting on $\mathcal{G}_i$}} \label{algo1:line:exact-count}
%\For{{\bf each} $v_0 \in$ $V_i$ \textbf{in parallel}} \Comment{\hl{a}} \label{algo3:line:v0}
%\For{{\bf each} $v_1 \in$ $N_i(v_0)$} \Comment{\hl{b}} \label{algo3:line:v1}
%\For{{\bf each} $v_2 \in$ $N_i(v_1)$} \Comment{\hl{c}} \label{algo3:line:v2}
%\State count++
%\EndFor
%\EndFor

==> algo-framework.tex <==
% Framework algorithm
% \begin{algorithm}[tb]
% \footnotesize
% \caption{Sansa Framework}
% \label{algo:framework}
% \begin{algorithmic}[1]

% \Input
% \State \makebox[4em][l]{$G(V,E)$} data graph
% \State \makebox[4em][l]{$P$} pattern graph
% \State \makebox[4em][l]{$\epsilon$} error bound
% \State \makebox[4em][l]{$k$} threshold
% \EndInput

% \State $C'$ $\leftarrow$ 0, $S \leftarrow\ \{ \}$
% \For{{\bf each} $ i \in$ $[0,n)$ \textbf{}}
% \If {$\texttt{thresholds}[v] \le n$}
%     $S \bigcup v $  
% \Else \ 
%     $C'$ += \Call{ExactCounting}{\dg, \pg, $v$}
% \EndIf

% \State $C'$ += \Call{ApproximateCount}{\dg, \pg, $S$} 
% \EndFor
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[tb]
\footnotesize
\caption{Sansa Framework}
\label{algo:framework}
\begin{algorithmic}
% \Input
% \State \makebox[4em][l]{\dg$(V,E)$} input data graph
% \State \makebox[4em][l]{\pg} input pattern graph
% \State \makebox[4em][l]{$\epsilon$} error bound
% \State \makebox[4em][l]{$\delta$} confidence
% \EndInput

% \Output
% \State \makebox[4em][l]{$C$} count of matches
% \EndOutput

%\item[]

\State $R \gets$ \Call{\hlg{InitSamplingRule}}{\dg, \pg, $\epsilon, \delta$}  \Comment{UDF}
%\If {ENABLE\_ELP = true} %\Comment{User Ddefined Flag}
  \State $R \gets$ \Call{{Profiling}}{\dg, \pg, $\epsilon$, $\delta$, $R$} 
  \Comment{$R$ is the sampling rule}
%\EndIf
%\State $\alpha \gets \frac{|U|}{\beta}$ \Comment{$\alpha$ is scale factor}
\State $N \gets R.N_s$
\For {$i \in [1,N]$}
    \State $H_i \gets$ \Call{\hlg{Sample}}{\dg, \pg, $R$} \Comment{mandatory UDF}
    \State $C_i \gets$ \Call{\hlg{Count}}{\dg, \pg, $H_i$} \Comment{mandatory UDF}
    %\State $C \gets C + C_i * \alpha$
\EndFor
%\State $\alpha \gets$ \Call {\hlb{GenScaleFactor}}{\dg, \pg, $\epsilon$, $R$} 
%\Comment{\hl{Not sure if this should be a UDF or not} \hl{-- Could be derived from definition of Sample?}}
\State $C \gets \sum C_i / N$ %\Comment{$\alpha$ is the scale factor}

\end{algorithmic}
\end{algorithm}

==> algo-graphzero-4cycle.tex <==
\begin{algorithm}[htb]
%\scriptsize
\footnotesize
\caption{Exact {\tt 4-cycle} counting in GraphZero~\cite{GraphZero}}
\label{algo:graphzero-4cycle}
\begin{algorithmic}[1]
  \For{{\bf each} vertex $v_1 \in$ \vs }  \Comment{\hlg{match $v_1$ to $u_1$}} \label{algo:dfs:for1}
    \For{{\bf each} vertex $v_2 \in$ \adj($v_1$)} \Comment{\hlg{match $v_2$ to $u_2$}} \label{algo:dfs:for2}
	  \If{$v_2\ge v_1$} break; \Comment{\hlg{symmetry breaking}} \label{algo:dfs:break1}
	  \EndIf
        \For{{\bf each} vertex $v_3 \in$ \adj($v_1$)} \Comment{\hlg{match $v_3$ to $u_3$}} \label{algo:dfs:for3} 
	  \If{$v_3\ge v_2$} break; \Comment{\hlg{symmetry breaking}} \label{algo:dfs:break2}
	  \EndIf
	  %\State $W \leftarrow$ \adj($v_1$) $\cap$ \adj($v_2$); \Comment{\hlg{set intersection: buffered in $W$}} \label{algo:dfs:buffer}
      %\For{{\bf each} vertex $v_3 \in W$} \Comment{\hlg{match $v_3$ to $u_3$}} \label{algo:dfs:for3}
      \For{{\bf each} vertex $v_4 \in $ \adj($v_1$) $\cap$ \adj($v_2$)} \Comment{\hlg{match $v_4$ to $u_4$}} \label{algo:dfs:for4}
	      \If{$v_4\ge v_0$} break; \Comment{\hlg{symmetry breaking}} \label{algo:dfs:break3}
	      \Else $ $ count ++; \Comment{\hlg{do the counting}}
	      \EndIf
	    \EndFor
	  \EndFor
    \EndFor
  \EndFor
\end{algorithmic}
\end{algorithm}

==> algo-graphzero-diamond.tex <==
\iffalse
\begin{lstlisting}[
float=tp,floatplacement=t,
xleftmargin=0.2in,
linewidth=6cm,
label={lst:dfs},
basicstyle=\ttfamily\footnotesize,
language=C++, 
abovecaptionskip=0pt,
%frame = trBL, 
firstnumber = last, 
escapeinside={(*@}{@*)},
escapeinside={(*}{*)},
morekeywords = {define, vertex, final},
caption = {Pseudo code for finding {\tt diamond} in DFS order}]
for (each (*$v_0 \in V$*) in parallel)
  for (each (*$v_1 \in$*) N((*$v_0$*)))
    if ((*$v_1>v_0$*)) break;
    for (each (*$v_2 \in$*) N((*$v_0$*)))
      for (each (*$v_3 \in$*) N((*$v_1$*))(*$\cap$*) N((*$v_2$*)))
        if ((*$v_3$*)>(*$v_2$*)) break;
        count ++;
\end{lstlisting}
\fi

\begin{algorithm}[t]
%\scriptsize
\footnotesize
\caption{GraphZero pseudo code for {\tt diamond} pattern}
\label{alg:graphzero-diamond}
\begin{algorithmic}[1]
  \For{{\bf each} vertex $v_1 \in$ \vs }  \Comment{\hlg{match $v_1$ to $u_1$}} \label{algo:dfs:for1}
    \For{{\bf each} vertex $v_2 \in$ \adj($v_1$)} \Comment{\hlg{match $v_2$ to $u_2$}} \label{algo:dfs:for2}
	  \If{$v_2\ge v_1$} break; \Comment{\hlg{symmetry breaking}} \label{algo:dfs:break1}
	  \EndIf
	  \State $W \leftarrow$ \adj($v_1$) $\cap$ \adj($v_2$); \Comment{\hlg{set intersection: buffered in $W$}} \label{algo:dfs:buffer}
      \For{{\bf each} vertex $v_3 \in W$} \Comment{\hlg{match $v_3$ to $u_3$}} \label{algo:dfs:for3}
      \For{{\bf each} vertex $v_4 \in W$} \Comment{\hlg{match $v_4$ to $u_4$; $W$ is reused}} \label{algo:dfs:for4}
	      \If{$v_4\ge v_3$} break; \Comment{\hlg{symmetry breaking}} \label{algo:dfs:break2}
	      \Else $ $ count ++; \Comment{\hlg{do the counting}}
	      \EndIf
	    \EndFor
	  \EndFor
    \EndFor
  \EndFor
\end{algorithmic}
\end{algorithm}

==> algo-main.tex <==
\begin{algorithm}[tb]
\footnotesize
\caption{Approximate Count with Color Sparsification}
\label{alg1:main}
\begin{algorithmic}[1]

\Input
\State \makebox[4em][l]{$G(V,E)$} data graph
\State \makebox[4em][l]{$P$} pattern graph
\State \makebox[4em][l]{$c$} number of colors for error bound from ELP

\EndInput

\Output
\State \makebox[4em][l] {$C$} estimated count
\EndOutput

\State count $\leftarrow$ 0


\State $colors$[] = \Call{Color}{$V$, $c$} 
\Comment{\hl{Color the graph using $c$ colors}}  \label{algo3:line:color}

%\While{error $> \epsilon$} \label{algo3:line:while}

%\tikzmk{A}
\For{{\bf each} $ i \in$ $[0,k)$ \textbf{}}
\State $V_i \leftarrow \{v | v \in V \& colors[v]=i\}$   \Comment{\hl{All the vertices with color $i$}}
\State Generate an induced subgraph $\mathcal{G}_i=(V_i, E_i)$  \label{algo3:line:genSubgraph}

\State count += \Call{ExactCounting}{$\mathcal{G}_i$, $P$} \Comment{\hl{Exact counting on $\mathcal{G}_i$}} \label{algo1:line:exact-count}
\EndFor

\State $C$ $\leftarrow$ \Call{Scale}{count, $P$, $k$}

%\EndFor
%\EndWhile
\end{algorithmic}
\end{algorithm}


==> algo-ns-base.tex <==

\begin{algorithm}[htb]
\footnotesize
\caption{\NS-base for \texttt{4-cycle}}
\label{algo:ns-4cycle}
\begin{algorithmic}[1]

\For{{\bf each} sampler $i \in$ [1, $N_s$]} \label{algo:ns:line:each-sampler}

%\State $C_i \gets 0$  
\State $e(v_0, v_1) \gets$  \Call{sample}{$\mathcal{E}$} , $\alpha \gets 0$ \Comment{\hlg{sample} an edge $(v_0, v_1)$} \label{algo:ns-base:line:sample-first-edge}
%\State $S_1 \gets$ \{$v_0$, $v_1$\}
\State $A \gets$ $N(v_0) \cup N(v_1)$ - \{$v_0$, $v_1$\}
\Comment{\hlg{set union and difference}}  \label{algo:ns-base:line:v2} 
\If{|A| = 0} break\EndIf \label{algo:ns-base:line:breakA} %\Comment{failed, early exit}
\State $v_2 \gets$ \Call{sample}{$A$} \Comment{\hlg{sample} node $v_2$ from set $A$} \label{algo:ns-base:line:sample-v2} 
\State $B \gets$ $N(v_0) \cup N(v_2)$ - \{$v_0, v_1, v_2$\} \Comment{\hlg{set union and difference}} \label{algo:ns-base:line:v3} 
\If{|B| = 0} break\EndIf \label{algo:ns-base:line:breakB} %\Comment{failed, early exit}
\State $v_3\gets$ \Call{sample}{$B$}  \Comment{\hlg{sample} node $v_3$ from set $B$} \label{algo:ns-base:line:sample-v3}
%\State VertexSet vs4 = $N(v_1)$ - $vs02$
\If{edge $(v_0, v_3)$ exist in \dg} \Comment{check closure}
\State $\alpha \gets m * |A| * |B| / 16$  \Comment{scaling factor}
\EndIf
\EndFor
%\State $C' = \sum C_i / N_s$ is the estimated count  \label{algo:ns:line:average}
\end{algorithmic}
\end{algorithm}

==> code-API.tex <==
\begin{lstlisting}[
float=*,
floatplacement=tb,
xleftmargin=0in,
linewidth=18cm,
label={listing:code-api},
basicstyle=\ttfamily\footnotesize,
language=C++, 
abovecaptionskip=0pt,
frame = trBL, 
firstnumber = last, 
escapeinside={(*@}{@*)},
escapeinside={(*}{*)},
%mathescape=true,
morekeywords = {Vector, Bool, Integer, Float, Graph, Vertex, Edge, VertexSet, EdgeSet, Cond},
caption = {API helper functions}]
EdgeSet SampleEdges(Graph g, Float p = 0) // sample a set of edges in the Graph g with a probability p.
VertexSet SampleNeighbor(VertexSet Q, Float p = 0) // sample neighbors in Q's neighborhood
EdgeSet SampleNeighbor(EdgeSet R, Float p = 0) // sample neighbors in R's neighborhood
Graph Color(Graph g, Integer k) // randomly color each vertex in the graph with k colors 
Graph GenSubgraph(Graph g, VertexSet Q, EdgeSet R) // generate a subgraph from Q or R, Q (*$\subseteq$*) g.V, R (*$\subseteq$*) g.E
Bool CheckClosure(Graph h, Graph P, Graph g) // check closure of h for pattern P exist in Graph g.
Integer ExactCount(Graph g, Graph P, Cond constraints={}) // count exactly the number of matches of P
VertexSet Intersect(VertexSet Q1, ... VertexSet Qn) // find the intersection of n vertex sets.
VertexSet Union(VertexSet Q1, ... VertexSet Qn) // find the union of n vertex sets.

\end{lstlisting}

% Edge SampleEdge(Graph g) // randomly sample an edge in the Graph g.


% EdgeSet SampleNeighborEdges(EdgeSet e, Float p) // randomly sample many edges, incident to each edge in e, with probability p.

% Vertex SampleNeighborVertex(Vertex v) // randomly sample a neighboring vertex in vertex v's neighborhood.

% Edge SampleNeighborEdge(Vertex v) // randomly sample a neighboring edge in vertex v's neighborhood.


%// and return a labeled graph, with some color as the label for each vertex



==> elp.tex <==






==> read-k.tex <==



Formally, let $Y_1 \dots Y_C$ be the random variables that represent the existence of matches, where $Y_i = 1$ if the match $M_i$ was preserved in the sparsified graph and $Y_i = 0$ if any of the edges within the match were removed.
As $Y_i$ is not independent, this means that we can not use the standard Chernoff bound to tightly bound error. We could use Chebyshev bound 
%(if we consider the covariance between each instance of the pattern in our calculation of the variance), 
but this is not a tight enough bound to be useful in practice. 

We use the `read-$k$' extension of Chernoff bounds~\cite{read-k}. 
The key idea is to map the dependent random variables $Y_i$ to a set of independent random variables $X_i$, and derive a bound from them.
The `read-$k$' extension gives the same bound as that of the standard Chernoff bound, except that the exponent is divided by $k$, where $k$ is the maximum number of $Y_i$ mapped to any $X_j$.

In our case, the edges are removed randomly. 
Let $X_1 \dots X_m$ be random variables for each of the $m$ edges in \dg, where $X_i = 1$ if the edge was preserved and $X_i = 0$ if the edge was removed. We can see each edge has the probability $\hat{p}$ of being preserved and this probability is independent of any other edge, $X_j$, even if they may share one endpoint.
Then $Y_i$ is dependent on exactly $l$ of the $X_1 \dots X_m$ edges, which are the specific edges that make up that match $M_i$. 
We define $\gamma$ as the maximum number of matches (of \pg) incident to an edge.
Thus, we can apply the `read-$k$' extension with $k = \gamma$, which gives the following theorem. 

\begin{theorem}
Given a data graph \dg and a pattern \pg, 
$p \geq \frac{-3\cdot\ln(\delta / 2)\gamma}{\epsilon^2 \cdot C }$
obtains an $\epsilon$-$\delta$ estimation of $C$, the number of matches of \pg in \dg.
\end{theorem}

So in order to determine a good value for $p$, we need to estimate $C$ and $\gamma$,
which is done by the fast profiling~\cref{subsect:profiler} on the graph \dg.
We assume that $\hat{p}$ is not very sensitive to $C$ and $\gamma$. So we don't need a very accurate estimation of $C$ and $\gamma$ in this profiling.

==> region-split.tex <==
\subsection{Sparse-Dense Region Split}

Sansa's proposed framework revolves around splitting the graph into dense and sparse regions, and then performing an approximate count using color sparsification in the dense regions and exact counting in the sparse regions.

Sansa leverages a neighborhood degree-thresholding system in order to partition the graph into dense and sparse regions as seen in  \cref{alg1:framework}. Such a thresholding scheme has been seen in previous work specific to cliques \cite{kclique:2022}, but Sansa generalizes it to a pattern-agnostic system. In dense regions, exact counting can be very expensive, particularly with dense or large patterns such as cliques. Therefore, Sansa can aggressively use sampling methods in these dense regions while maintaining accuracy and see large performance benefits. In sparse regions, an exact counting solution can still be leveraged on the original graph where a sampling method would be ineffective in finding a representative number of instances of the target pattern.

The thresholding occurs based on a degree-threshold constant, $k$, which is set based on the input target pattern. For cliques, $k$ is the degree of the clique, but for other patterns, this $k$ is adjusted based on the exact counting algorithm used.

Because Sansa's leverages this framework, it is not restricted to dense settings as Arya and ASAP are, mitigating the "needle-in-the-hay" problems. The thresholding system is particularly useful as applications may not be able to easily determine if their input graph and target pattern are sparse or dense.

==> subg-gen.tex <==
\subsection {Efficient Coloring and Subgraph Generation}

Sansa could be tuned to generally use any algorithm to take a subgraph sample as an overhead step as long as a corresponding scaling algorithm is applied.

We implemented and tested Sansa with Color Sparsification, Edge Sparsification, and N-Random-Tree sampling as several subgraph sampling methods.

\subsubsection{Color Sparsification}

Color sparsification has seen use in other pattern-specific domains such as five-cycles \cite{Five-Cycle}, butterflies, and triangles. However, the technique can be adjusted to be generalizable to a multi-pattern system. Color sparsification involves randomly assigning each node in the graph a random color, and then only preserving edges where the two end vertices share a color. Furthermore, with overhead-reducing optimizations Sansa's color-sparsification step is relatively inexpensive and can be re-used across many different patterns even with different granularities of spasification, $c$.

For speed improvements and to decrease the overhead cost of the color spasification step, Sansa leverages a dynamic color-merge-split adaptation to the Compressed Sparse Row (CSR) graph data structure. The color-merge-split stores an additional dynamic pointer to the end of the colored edge lists, which are sorted in accordance to which colors they belong to as demonstrated in \cref{fig:csr}. This allows for dynamic color group merging/splitting by adjusting the end pointer in the CSR. 


\begin{figure}[h!]
\centering
\includegraphics[width=80mm]{figures/diagram.png}
\caption{Color-Merge-Split CSR}
\label{fig:csr}
\end{figure}

This flexible coloring method allows for the computation of several colorings at once for time saving at the cost of additional overhead. This allows for the ELP to calculate several estimations at once without re-running the coloring overhead step.

The overhead time of this coloring time can be combined with the overhead time of loading in the graph and any other pre-processing needed for the exact counting method. One dynamic coloring can then be used for counts of different patterns. 

The coloring process always take $O(|V| + |E|)$ time and requires $O(|V| + |E|/c*k)$ storage where $c$ is the number of colors and $k$ is the number of colorings to preform.

\input{algo-main}

The scaled count of patterns within a color partition is a $1-\epsilon$ unbiased estimator of the true count of instances of patterns in the graph.

The count obtained in the color-sparsified subgraph sample is then scaled in accordance to the following equation, where Y is the scaled output count, $c$ is the number of colors, $k$ is the number of nodes in target pattern, and $C$ is the observed count.

$$Y = C*(1/c)^{-(k-1)}$$

This scale factor represents the probability that fixing one vertex of the target pattern, that the other $k-1$ vertices have the same color as the first vertex, which occurs with probability $1/c$.


\subsection{Sub-Graph Sampling Compared Neighbor Sampling}

Arya and ASAP both use variations of random neighbor sampling to build up edges and test instances of a pattern whereas Sansa uses a single sub-graph sample.

Sparsification, which is either edge sparsification (in which each edge is randomly preserved with probability $p$) or color sparsification (in which each node is colored with one of $c$ colors), creates a single random subgraph sample. Sansa takes one large sub-graph sample and performs an exact count, whereas neighbor sampling methods take many target-pattern-sized edge samples.

Therefore, for neighbor sampling methods, the counting process is embedded in the sampling process and exact-counting optimization may not be possible to apply. For example, because Arya is based around stars and odd-length cycle decomposition, it struggles with patterns that do not have favorable decompositions (such as 9-cliques). The sampling process therefore restricts the flexibility of counting step of the system whereas Sansa's is pattern-agnostic.

One benefit of using specifically color sparsification, is that the scaling term is proportional to the number of nodes in the pattern instead of the number of edges. Whereas edge-based sparsification and sampling, the algorithm is limited to finding edge-induced counts of the pattern. Color sparsification works in both edge-induced and vertex-induced settings.

==> table_sysperf.tex <==
\begin{table}[t]
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{r|rrr|rrr|rr}
% \Xhline{2\arrayrulewidth}
\multicolumn{1}{c|}{\textbf{Pattern}} & \multicolumn{3}{c|}{\textbf{Triangle}} & \multicolumn{3}{c|}{\textbf{4-clique}} & \multicolumn{2}{c}{\textbf{6-clique}}    \\ 
\hline
\multicolumn{1}{c|}{\textbf{Graph}} & \texttt{Lj} & \texttt{Tw} & \texttt{Fr} & \texttt{Lj} & \texttt{Tw} & \texttt{Fr} & \texttt{Lj} & \texttt{Fr} \\
\hline

% \sys (NS) & 0.005 (NS) & 0.252 (NS) & 0.101 (NS) & 0.038 (NS) & 64.9 (NS) & 0.038 (NS) & 0.184 (NS) &10.8 (GS)  \\    
\sys & \textbf{0.005}  & \textbf{0.25} & \textbf{0.10}  & \textbf{0.04}  & \textbf{6.5}  & \textbf{0.038}  & \textbf{0.20}  &  \textbf{10.8}* \\
% \sys (\GS) & $\uparrow$ & $\uparrow$ & $\uparrow$ & $\uparrow$ & $\uparrow$ & $\uparrow$ & $\uparrow$ &10.8   \\
Arya & 0.12       & 9.5      & 1.3      & 0.06       & 16.2    & 65.7     & 90.6      &657.7         \\
GraphZero & 0.15      & 23.3         & 20.3        & 5.6      & 1105.7     & 22.8      & 26254.4      &  53.8  \\
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\caption{\small $k$-clique running time (s) with 10\% error. 
TO: timed out. (*) Indicates \GS engine selected, otherwise \NS is selected.}
\label{tab:clique}
\end{table}

\begin{table}[t]
\resizebox{.49\textwidth}{!}{
\begin{tabular}{r|rrr|rrr|rr}
%\Xhline{2\arrayrulewidth}
\multicolumn{1}{c|}{\textbf{Pattern}} & \multicolumn{3}{c|}{\textbf{5-path}} & \multicolumn{3}{c|}{\textbf{5-house}} & \multicolumn{2}{c}{\textbf{6-dumbbell}}    \\ 
\hline
\multicolumn{1}{c|}{\textbf{Graph}} & \texttt{Lj} & \texttt{Tw} & \texttt{Fr} & \texttt{Lj} & \texttt{Tw} & \texttt{Fr} & \texttt{Lj}  & \texttt{Fr}\\
\hline

%\sys & 0.169 (NS) & 3201.71 (NS) & 0.1483 (NS) & 0.00929 (NS)&       1296.7 (GS) & 2.48748 (NS) & 0.0139 (NS) &  2.93 (NS) \\

\sys & \textbf{0.17}  & \textbf{3201.7} & \textbf{0.15}  & \textbf{0.009} & \textbf{1296.7}* & \textbf{2.5} & \textbf{0.014}  &  \textbf{2.93}  \\
%\sys (\GS) & $\uparrow$ &$\uparrow$  &$\uparrow$  & $\uparrow$&       1296.7  & $\uparrow$ & $\uparrow$ &$\uparrow$   \\
Arya & 0.14 & {TO} & 1.11 & 0.28 &  {TO} & 4.33 & 0.10    & 3.00 \\
% Arya & 0.14356       &  {\bf TO}    & 1.11        & 0.27962 &  {\bf TO}    & 4.33232      & 0.10286    & 3.00122 \\
GraphZero & 195.9 & {TO} & {TO} & 45300.2 & {TO} & {TO} & {TO} & {TO}  \\
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\caption{\small Large non-clique pattern running time (s). 
TO: timed out.  (*) Indicates \GS engine selected.}
\label{tab:complex}
\end{table}

\begin{table}[t]
\centering
\resizebox{0.43\textwidth}{!}{
\begin{tabular}{r|rrr|rrr}
% \Xhline{2\arrayrulewidth}
\multicolumn{1}{c|}{\textbf{Pattern}} & \multicolumn{3}{c|}{\textbf{3-motif}} & \multicolumn{3}{c}{\textbf{4-motif}}   \\ 
\hline
\multicolumn{1}{c|}{\textbf{Graph}} & \texttt{Lj} & \texttt{Tw} & \texttt{Fr} & \texttt{Lj} & \texttt{Tw} & \texttt{Fr}\\
\hline

% \sys & 0.012 & 0.405 & 0.144 & 0.252 GS & 33.7 GS & 15.9 GS \\
\sys  & \textbf{0.01} & \textbf{0.41} & \textbf{0.14} & \textbf{0.25}*  & \textbf{33.7}*  & \textbf{15.9}* \\
% \sys (\GS) & $\uparrow$ &$\uparrow$  & $\uparrow$ & 0.25  & 33.7  & 15.9  \\
Arya &0.03 & 1.3 & 2.2 & 3.9 & 1224.9 & 78.8 \\
GraphZero & 1.4 & 67.7 & 65.4 & 1702.9 & {TO} &  35019.7 \\
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\caption{\small Motif counting running time (s) with 10\% error. 
TO: timed out. (*) Indicates \GS engine selected.}
\label{tab:motif}
\end{table}

\begin{table}[t]
\centering
\resizebox{0.35\textwidth}{!}{
\begin{tabular}{r|rr|rr|r}
% \Xhline{2\arrayrulewidth}
\multicolumn{1}{c|}{\textbf{Pattern}} & \multicolumn{2}{c|}{\textbf{triangle}} & \multicolumn{2}{c|}{\textbf{4-clique}} & \multicolumn{1}{c}{\textbf{5-house}}    \\ \hline
\multicolumn{1}{c|}{\textbf{Graph}} & \texttt{gsh} & \texttt{cw} & \texttt{gsh} & \texttt{cw} & \texttt{gsh}  \\ \hline
%\sys &0.900 (NS) &0.559 (NS) &1.05 (NS)  &1.17409 (NS) &4201.44 (GS) \\
\sys  & \textbf{0.90}  & \textbf{0.56}  & \textbf{1.1}  & \textbf{1.2} & \textbf{ 4201.4}* \\
% \sys (\GS) & $\uparrow$ & $\uparrow$ &  $\uparrow$ & $\uparrow$  &4201.4  \\
GraphZero & 76.4 & 52.4 & {TO} & {TO} & {TO} \\
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\caption{\small running time (s) on very large graphs. 
TO: timed out. (*) Indicates \GS engine selected.}
\label{tab:large}
\end{table}





==> vldb_block.tex <==

%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\pagestyle{\vldbpagestyle}
\begingroup\small\noindent\raggedright\textbf{PVLDB Reference Format:}\\
\vldbauthors. \vldbtitle. PVLDB, \vldbvolume(\vldbissue): \vldbpages, \vldbyear.\\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi}
\endgroup
\begingroup
\renewcommand\thefootnote{}\footnote{\noindent
This work is licensed under the Creative Commons BY-NC-ND 4.0 International License. Visit \url{https://creativecommons.org/licenses/by-nc-nd/4.0/} to view a copy of this license. For any use beyond those covered by this license, obtain permission by emailing \href{mailto:info@vldb.org}{info@vldb.org}. Copyright is held by the owner/author(s). Publication rights licensed to the VLDB Endowment. \\
\raggedright Proceedings of the VLDB Endowment, Vol. \vldbvolume, No. \vldbissue\ %
ISSN 2150-8097. \\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi} \\
}\addtocounter{footnote}{-1}\endgroup
%%% VLDB block end %%%

%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\ifdefempty{\vldbavailabilityurl}{}{
\vspace{.3cm}
\begingroup\small\noindent\raggedright\textbf{PVLDB Artifact Availability:}\\
The source code, data, and/or other artifacts have been made available at \url{\vldbavailabilityurl}.
\endgroup
}
%%% VLDB block end %%%
